"The Data Says Otherwise"-Towards Automated Fact-checking and Communication of Data Claims

Fact-checking data claims requires data evidence retrieval and analysis, which can become tedious and intractable when done manually. This work presents Aletheia, an automated fact-checking prototype designed to facilitate data claims verification and enhance data evidence communication. For verification, we utilize a pre-trained LLM to parse the semantics for evidence retrieval. To effectively communicate the data evidence, we design representations in two forms: data tables and visualizations, tailored to various data fact types. Additionally, we design interactions that showcase a real-world application of these techniques. We evaluate the performance of two core NLP tasks with a curated dataset comprising 400 data claims and compare the two representation forms regarding viewers' assessment time, confidence, and preference via a user study with 20 participants. The evaluation offers insights into the feasibility and bottlenecks of using LLMs for data fact-checking tasks, potential advantages and disadvantages of using visualizations over data tables, and design recommendations for presenting data evidence.

==> sections/0-abstract.tex <==

\begin{abstract}


Fact-checking data claims requires data evidence retrieval and analysis, which can become tedious and intractable when done manually. This work presents \sys{}, an automated fact-checking prototype designed to facilitate data claims \emph{verification} and enhance data evidence \emph{communication}. For verification, we utilize a pre-trained LLM to parse the semantics for evidence retrieval. To effectively communicate the data evidence, we design representations in two forms: data tables and visualizations, tailored to various data fact types. Additionally, we design interactions that showcase a real-world application of these techniques.  We evaluate the performance of two core NLP tasks with a curated dataset comprising 400 data claims and compare the two representation forms regarding viewers' assessment time, confidence, and preference via a user study with 20 participants. The evaluation offers insights into the feasibility and bottlenecks of using LLMs for data fact-checking tasks, potential advantages and disadvantages of using visualizations over data tables, and design recommendations for presenting data evidence.






% \noindent\todo{Add abstract}\\
% \noindent\todo{Discuss the CCS Concepts and Keywords}\\

\end{abstract}

%%
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
%%
\begin{CCSXML}
<ccs2012>
   <concept>
       <concept_id>10003120.10003121.10003126</concept_id>
       <concept_desc>Human-centered computing~HCI theory, concepts and models</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10003120.10003145.10011769</concept_id>
       <concept_desc>Human-centered computing~Empirical studies in visualization</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10002951.10003317.10003325</concept_id>
       <concept_desc>Information systems~Information retrieval query processing</concept_desc>
       <concept_significance>300</concept_significance>
       </concept>
 </ccs2012>
\end{CCSXML}

\ccsdesc[500]{Human-centered computing~HCI theory, concepts and models}
\ccsdesc[500]{Human-centered computing~Empirical studies in visualization}
\ccsdesc[300]{Information systems~Information retrieval query processing}

%%
%% Keywords. The author(s) should pick words that accurately describe
%% the work being presented. Separate the keywords with commas.
\keywords{automated fact-checking, information visualization, data-driven storytelling}

==> sections/commands.tex <==
%!TEX root = proceedings.tex

%% Note: Relevant packages added for the contents of this file
%% Please include a comment describing the purpose of each new package
% \usepackage{xargs}      % Used for new commands with optional arguments


%% Note: Preprint notice to add to title when sharing early version of paper
\newcommand{\preprintNotice}{\textcolor{red}{Preprint: Currently under review. Please do not redistribute.}}

%% Note: New command for mentioning the system name
\newcommand{\sys}{\textit{Aletheia}}

%% Note: Some commands for spacing Latin letters/abbreviations
\newcommand{\ie}{{i.e.,}\xspace}
\newcommand{\eg}{{e.g.,}\xspace}
\newcommand{\etal}{{et~al\xperiod}\xspace}
\newcommand{\aka}{{a.k.a.}\xspace}
\newcommand{\etc}{{etc\xperiod}\xspace}

%% Note: Commands for custom styling of participant quotes
\newcommand{\myquote}[1]{\emph{``#1''}}                         % Italic text in quotation marks
\newcommand{\myquoteparticipant}[2]{\emph{``#1''}~(#2)}         % Italic text in quotation marks AND P# with non-breaking space
\newcommand{\mylongquote}[1]{\begin{quote}\emph{#1}\end{quote}} % Block quote in italics, no quotation marks or P#

%% Note: Commands for custom styling of bold, inline paragraph headings
\newcommand{\parHeading}[1]{\vspace{8px}\noindent{\textbf{#1}}}

%% Note: Custom colors for in-paper comments
\definecolor{lightpink}{RGB}{237,157,202}
\definecolor{lightred}{RGB}{210,121,121}
\definecolor{lightorange}{RGB}{230,170,50}
\definecolor{lightgold}{RGB}{210,194,121}
\definecolor{lightgreen}{RGB}{121,210,121}
\definecolor{lightaqua}{RGB}{121,206,210}
\definecolor{lightblue}{RGB}{121,124,210}
\definecolor{lightpurple}{RGB}{153,102,255}
\definecolor{red}{RGB}{178,34,34}
\definecolor{gray}{RGB}{166,166,166}
\definecolor{peach}{RGB}{255,218,185}

\definecolor{Amber}{RGB}{255,190,11}
\definecolor{Pantone}{RGB}{251,86,7}
\definecolor{Rose}{RGB}{255,0,110}
\definecolor{Violet}{RGB}{131,56,236}
\definecolor{Azure}{RGB}{58,134,255}
\definecolor{mypurple}{RGB}{131,56,236}
\definecolor{myred}{RGB}{251,86,7}
\definecolor{mydarkred}{RGB}{252,102,32}
\definecolor{mydarkpurple}{RGB}{144,77,238}

\newcommand{\purpleBox}[2][0.8]{%
  \transparent{#1}\colorbox{mypurple}{#2}
}

\newcommand{\redBox}[2][0.8]{%
  \transparent{#1}\colorbox{myred}{#2}
}

\captionsetup{labelfont=normalfont,textfont=normalfont}



% [{"name":"Amber","hex":"ffbe0b","rgb":[],"cmyk":[0,25,96,0],"hsb":[44,96,100],"hsl":[44,100,52],"lab":[81,11,82]},{"name":"Orange (Pantone)","hex":"fb5607","rgb":[251,86,7],"cmyk":[0,66,97,2],"hsb":[19,97,98],"hsl":[19,97,51],"lab":[59,60,68]},{"name":"Rose","hex":"ff006e","rgb":[255,0,110],"cmyk":[0,100,57,0],"hsb":[334,100,100],"hsl":[334,100,50],"lab":[54,83,14]},{"name":"Blue Violet","hex":"8338ec","rgb":[131,56,236],"cmyk":[44,76,0,7],"hsb":[265,76,93],"hsl":[265,83,57],"lab":[44,66,-78]},{"name":"Azure","hex":"3a86ff","rgb":[58,134,255],"cmyk":[77,47,0,0],"hsb":[217,77,100],"hsl":[217,100,61],"lab":[57,18,-67]}]

%% NOTE: Table color/style commands
\newcommand{\claimSpecColor}[3][1=]{ %
    % \textcolor{#3}{#1} % Change the color of the first argument (text value)
    \setulcolor{#3}{\ul{#1~{#2}}} % Underline the first argument (text value)
    %\textcolor{#3}{#2} % Change the color of the second argument (variable)
    % ~{#2} % Show the second argument in black (variable)
}
\newcommand{\claimSpecColorNEW}[3][1=]{\setulcolor{#3}{\ul{#1}}}
\newcommand{\claimVarStyle}[1]{\texttt{\{#1\}}}
\newcommand{\claimVarStyleNEW}[1]{\textnormal{#1}}

%% Note: General TODO and cut commands
\newcommand{\todo}[1]{\textcolor{red}{[TODO] \emph{#1}}}
\newcommand{\cut}[1]{\textcolor{red}{\st{#1}}}
\newcommand{\rv}[1]{\textcolor{black}{#1}}

%% Note: Labeled in-paper comments for paper authors (with and without underlined text)
% \newcommandx{\guest}[3][1=]
%     {\setulcolor{lightorange}{\ul{#1}} \textcolor{lightorange} %% Usage: \guest[Underline]{Name}{Comment}
%     {[\textbf{#2:} #3]}}

% \newcommandx{\yu}[2][1=] 
%     {\setulcolor{orange}{\ul{#1}} \textcolor{orange}   %% Usage: \jane[(optionally) underline text]{With a comment.}
%     {[\textbf{Yu:} #2]}}

% \newcommandx{\jane}[2][1=] 
%     {\setulcolor{lightgreen}{\ul{#1}} \textcolor{lightgreen}   %% Usage: \jane[(optionally) underline text]{With a comment.}
%     {[\textbf{Jane:} #2]}}
    
% \newcommandx{\shunan}[2][1=]{\setulcolor{teal}{\ul{#1}} \textcolor{teal}{[\textbf{Shunan:} #2]}}
% \newcommandx{\ryan}[2][1=]{\setulcolor{blue}{\ul{#1}} \textcolor{blue}{[\textbf{Ryan:} #2]}}

% \newcommandx{\victor}[2][1=]{\setulcolor{red}{\ul{#1}} \textcolor{red}{[\textbf{Victor:} #2]}}

    
%% Note: Section status badges to label which sections are ready (or not) for feedback 
\newcommand{\badge}[2]{\colorbox{#1}{\textcolor{white}{\textsc{#2}}}}
\newcommand{\headerBadge}[2]{
  \vspace{-15px}                  % Move badge into header
  \hspace*{\fill}                 % Align badge right
  \badge{#1}{#2}                  % Create badge
  \vspace{4px}\linebreak\noindent % Spacing for first paragraph
}
\newcommand{\complete}{\headerBadge{lightpurple}{complete}}
\newcommand{\feedbackProvided}{\headerBadge{lightgreen}{feedback provided}}
\newcommand{\readyForFeedback}{\headerBadge{lightorange}{ready for feedback}}
\newcommand{\underRevision}{\headerBadge{lightred}{actively under revision}}
\newcommand{\incomplete}{\headerBadge{red}{missing or incomplete}}



==> sections/packages.tex <==
\usepackage{tabularx}
\usepackage{graphicx}
\usepackage{array}
\usepackage{booktabs}  % for \toprule, \bottomrule
\usepackage{color}     % for \color
\usepackage{multirow}
\usepackage{makecell}
\usepackage{colortbl} 
\usepackage{enumitem}
\usepackage{subcaption}
\usepackage{dirtytalk}
\usepackage{soul} 
\usepackage{xcolor} 
% \usepackage[table]{xcolor} 
\usepackage{xspace}     % Used for abbreviation spacing
\usepackage{xpunctuate} % Used for abbreviation spacing
\usepackage{natbib}
\usepackage{transparent}
\usepackage{tikz}
\usepackage{setspace}   % Used to update the spacing of the text in table 1 (10 data fact types)


\renewcommand{\sectionautorefname}{Section}
\renewcommand{\subsectionautorefname}{Subsection}

\newif{\ifhidecomments}
  \hidecommentsfalse 
\hidecommentstrue
\ifhidecomments
    % \newcommand{\yu}[1]{}
    \newcommand{\Shunan}[1]{}
    % \newcommand{\John}[1]{}

\else
    % \newcommand{\yu}[1]{\textbf{\small\sffamily{\textcolor{orange}{[#1 -- yu]}}}}
    \newcommand{\shunan}[1]{\textbf{\small\sffamily{\textcolor{DarkBlue}{[#1 -- Shunan]}}}}
    % \newcommand{\john}[1]{\textbf{\small\sffamily{\textcolor{brickred}{[#1 -- John]}}}}
  \fi
\newcommand{\edit}[1]{{\textcolor{editCol}{#1}}}
\newcommand{\mask}[1]{{\textcolor{maskCol}{#1}}}


\usepackage{listings}

% Define JSON highlighting
\lstdefinestyle{jsonstyle}{
    basicstyle=\ttfamily\tiny\setstretch{0.8},
    keywordstyle=\color{blue},
    stringstyle=\color{red},
    numberstyle=\color{purple},
    commentstyle=\color{gray},
    breaklines=true,
    breakatwhitespace=false,
    showstringspaces=false,
    % frame=single,
    morestring=[b]",
    morecomment=[s]{/*}{*/},
    morecomment=[l]//,
    morekeywords={true,false,null},
    literate=
        *{:}{{{\color{blue}:}}}{1}
        {,}{{{\color{blue},}}}{1},
    aboveskip=5pt,
    belowskip=5pt,
    xleftmargin=0pt,
    xrightmargin=0pt,
}


\lstdefinelanguage{json}{
   morestring=[b]",
   morestring=[d]'
}

\lstdefinestyle{customjson}{
   backgroundcolor=\color{white}, 
   basicstyle=\ttfamily\footnotesize, 
   breakatwhitespace=false,         
   breaklines=true,                 
   captionpos=b,                    
   keepspaces=true,                 
   numbers=left,                    
   numbersep=5pt,                  
   showspaces=false,                
   showstringspaces=false,
   showtabs=false,                  
   tabsize=2,
   language=json,
   stringstyle=\color{blue},
   keywordstyle=\color{purple}
}

\definecolor{revisioncolor}{rgb}{0.0, 0.0, 1.0}

